Multi-Domain Image-to-Image Translation with Adaptive Inference Graph

In this work, we address the problem of multi-domain image-to-image translation with particular attention paid to computational cost. In particular, current state of the art models require a large and deep model in order to handle the visual diversity of multiple domains. In a context of limited computational resources, increasing the network size may not be possible. Therefore, we propose to increase the network capacity by using an adaptive graph structure. At inference time, the network estimates its own graph by selecting specific sub-networks. Sub-network selection is implemented using Gumbel-Softmax in order to allow end-to-end training. This approach leads to an adjustable increase in number of parameters while preserving an almost constant computational cost. Our evaluation on two publicly available datasets of facial and painting images shows that our adaptive strategy generates better images with fewer artifacts than literature methods

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> letter.tex <==
%\onecolumn
%\begin{figure*}[tp]
\begin{strip}
\begin{minipage}{1.0\linewidth}
\centering
\Huge  Multi-Domain Image-to-Image Translation with Adaptive Inference Graph: Author's Response
\end{minipage}
%\end{figure*}
\end{strip}


\vspace{1.5cm}
First of all we want to thank the reviewers for their work. We appreciate the comments and proposals made by the reviewers. We have thoroughly reviewed the document accordingly, and we hope that it substantially improved the initial submission.
In relation to the writing, we introduced clarifications and corrections throughout the document. We hope that all these modifications satisfy the reviewers. 
Below, we provide precise answers to the questions and issues raised by the reviewers.\\


\noindent\shadowbox{\textbf{Reviewer 2 }}

\noindent\textbf{R2-1. The lack of sufficient information to allow replication
studies. To allow reproducible research, the source code
should be provided. I'd suggest providing the end-to-end
pipeline.
}
The code will be available online upon acceptance. 

\noindent\textbf{R2.2. Given a large amount of GANs, it will be valuable to
compare different and more recent approaches.}
First, note that none of these recent works address the problem of translation with limited resources. Second, recent approaches such as DRIT~\cite{lee2018diverse}, MUNIT~\cite{Huang_2018_ECCV} or MSGAN~\cite{MSGAN} address the problem of translation between pairs of domains and focus mostly on increasing the diversity of the generated images. On the contrary, in this work, we address the problem of multi-domain translation in the low resource regime. In this context, adapting these methods by having multiple networks is not suitable. More specific manners to adapt these methods to multiple domains would require substantial modifications and this could be done in a subsequent publication. At the time of the submission, ComboGAN and StarGAN were the only works for multi-domain translation. This discussion is now included in the experimental section. Note that, recently, a second version of StarGAN, named StarGAN V2 \cite{choi2020starganv2}, has been published at CVPR 2020. However, CVPR 2020 proceedings were not available at submission time.

\noindent\textbf{R2.3. There are some errors/typos }%, among which a couple that I took note of are:
We thank the reviewer for this careful reading. We corrected all the typos and double-check the second version. \\



\noindent\shadowbox{\textbf{Reviewer 3}}

\noindent\textbf{R3-1. The work deftly can use a rewriting and
  comb-through.}
We thank you for the careful reading. We corrected all the typos and further checked writing.

 \noindent\textbf{R3-2. While the results of qualitative study is
immersive an interesting, the correlation with use of FID
is interesting but not well-motivated. also it is not clear
what those distance measures mean and are those differences
statistically significant.} First, FID is a widely used metric \cite{park2019SPADE,choi2020starganv2,MSGAN}. Despite its arguable assumptions, FID is consider as one of the best metrics for measuring distances between image distributions since it correlates human perception. Regarding the statistical significance of the result, we want to highlight that \textit{Ada$^2$Net} outperforms every competitor methods and baselines for every single painter in both Tables~\ref{table:FID_sota} and~\ref{table:FID_Ablation}. To further show the superiority of our approach, we added the standard deviations in both tables.   

 
\noindent\textbf{R3-3. All in all the contribution is
  interesting albeit incremental.} We do not agree on this point. We claim that our work is highly novel in two main aspects. First, this is the first work that addresses the problem of image-to-image translation with a specific focus on limited resources. Second, to the best of our knowledge, \textit{Ada$^2$Net} is the first network for an image generation task with an  architecture that is adapted on the fly at inference time.\\



\noindent\shadowbox{\textbf{Reviewer 4}}

\noindent\textbf{R4-1.The design of the proposed generator looks quite complex.
There are total seven different kinds of loss function to
train the generator, and different loss function has
different weight. Can author introduce how to select these
weights properly?} We agree that our method uses a high number of losses. However, these losses directly derive from StarGAN \cite{choi2018stargan} (Eqs. \eqref{eq:rec1}, \eqref{eq:rec2}, \eqref{eq:clas1} and \eqref{eq:clas2}) and from the MUNIT framework \cite{Huang_2018_ECCV} (Eqs. \eqref{eq:rec3}, \eqref{eq:rec4}). We clarified this point by improving the structure of Section~\ref{sec:training}. In our experiments, we simply used the weighting coefficients provided in the papers of StarGAN \cite{choi2018stargan} and MUNIT \cite{Huang_2018_ECCV}. We added this comment to the manuscript in Section~\ref{sec:exp}.


\noindent\textbf{R4-2. In the proposed method, authors used a classifier $C_d$
to predict the domain of an image. However, would the
performance of the classifier affect the training of the
generator? For example, a classifier without sufficient
training may lead to a failure of image translation.}
This domain-classifier was introduced in StarGAN \cite{choi2018stargan} and is not a contribution of our paper. Nevertheless, we added an experiment where we evaluate the impact of this classifier on the performance (See Fig.~\ref{fig:ablationlosses} and Tab.~\ref{table:FID_loss_Ablation}). These experiments show that this classifier is essential to obtain images that look similar to the target domain. Regarding the amount of training data, we note that the proposed model works well on the Painting-14 dataset that contains fewer images per domain than CelebA. 


\noindent\textbf{R4-3. In Fig. 4, authors provide results of ablation study on
CelebA dataset. Authors designed two baselines for ablation
study, i.e. \textit{No-AdaGraph} and \textit{Ada$^2$Net-label}. But authors
only compare the proposed generator with the baseline
\textit{No-AdaGraph}. It would be better to compare results with
baseline \textit{Ada$^2$Net-label} as well.}
This is a really good remark. We added this baseline in the experiments.

\noindent\textbf{R4-4. There are several typos in this paper.}
 We corrected these typos and further checked writing.\\

\noindent\shadowbox{
  \textbf{Reviewer 5}}

\noindent\textbf{R5-1. Not well-expressed.}
We corrected this typo.

\noindent\textbf{R5-2.	The loss proposed in formulation (10) and (11) is
mainly come from the intuition but lack the mathematical
support. And the loss function is too complex so that we
can not clarify the insight of the method.}
Following other reviewers' suggestions, we changed the structure of the section dedicated to training losses. We also added a reference to \cite{Huang_2018_ECCV} that provides mathematical support to our training scheme.
Concerning the insight, we completed the ablation study with additional experiments (See Section \ref{sec:exp}) that provide deeper understanding about the role of each loss term.  

\noindent\textbf{R5-3.	The legends of the Figure2 and Figure3 all have the
red underlines below them.}
We corrected this.

\noindent\textbf{R5-4.	The experiments settings are too simple}
We followed an experimental setting similar to StarGAN \cite{choi2018stargan} that is a well-established method. Besides, while only experiments on facial data are reported in \cite{choi2018stargan}, we perform experiments on both face and painting images. If the reviewer could provide more specific comments concerning the setting, we could include these comments in the final version.\\


\noindent\shadowbox{\textbf{Reviewer 6 }}\\
\noindent\textbf{R6-1. There is no justification for the disentanglement of
content information and style information. It is unclear
why the outputs of the content encoder and the style
encoder correspond to content information and style
information, respectively.}
Thank you for the comment. We made this point more clear in the new version (See Section~\ref{sec:overall}). Our network disentangles content and style information thanks to the way the style code is used. Indeed, the style code is used only in the Instance Normalization (IN) layers. In IN, the same affine transformation is applied at every tensor location (see \eqref{eq:IN}). Therefore, the style encoder extracts information that is not related to location and structure. Conversely, since reconstruction loss is employed, the content encoder encodes what cannot be reconstructed from the style code. %Note that, this use of IN is similar to \cite{huang2017arbitrary,Huang_2018_ECCV}.

\noindent\textbf{R6-2. In Figure 1, there are multiple 'gating' MLPs to
determine which residual function to use. It seems that
only one 'gating' MLP is enough. What is the purpose to
conduct the selecting process for $K$ times?}
It seems there is a confusion concerning the definition of $K$. As shown in Fig.\ref{fig:mask}, within an adaptive residual block a single MLP is used for the K convolution layers. However, assuming that we use $B$ adaptive residual blocks, we use $B$ different MLPs.
Using only a single MLP, instead of $B$, would imply that the same gate is used in each block. Therefore, only $K$ different network paths could be used. Conversely, with different MLP for each block, we obtain a total of $B\times K$ possible path. Therefore, the capacity of the network is much higher.  

\noindent\textbf{R6-3. The use of the classifier $C_d$ and the loss
$\mathcal{L}^{dis}_{cls}$ is unknown. Why do you need to
  predict the domain of a real image?} This classifier is used following an adversarial strategy. We train this classifier on the real images, such that, we can enforce that the generated images have a style similar to the real images of the targeted style. We added a comment in the manuscript to clarify this motivation (See right after Eq.~\eqref{eq:clas2}). 
Note that this classifier was introduced in StarGAN \cite{choi2018stargan} and that more details can be found in this paper.

\noindent\textbf{R6-4. In Figure 2, there is no origin images for comparison.}
The first column corresponds to the original image. 

\noindent\textbf{R6-5. It is unclear whether the loss items used in Eq. (10)
and Eq. (11) are all effective. In the ablation study,
authors can compare the result of the proposed architecture
when removing some loss items.}
We completed our ablation including this experiment. The additional experiments and their analysis can be found in Section~\ref{sec:ablationLoss}.




%% \twocolumn

